Ultra-faint dwarf galaxies: unveiling the minimum mass of the first stars

The non-detection of zero-metallicity stars in ultra-faint dwarf galaxies (UFDs) can be used to constrain the Initial Mass Function (IMF) of the first (PopIII) stars by means of a statistical comparison between available data and predictions from chemical evolution models. To this end we develop a model that follows the formation of isolated UFDs, calibrated to best reproduce the available data for the best studied system: Bo\"otes I. Our statistical approach shows that UFDs are the best suitable systems to study the implications of the persisting non-detection of zero-metallicity stars on the PopIII IMF, i.e. its shape, the minimum mass ($m_{min}$), and the characteristic mass ($m_{ch}$). We show that accounting for the incomplete sampling of the IMF is essential to compute the expected number of long-lived PopIII stars in inefficiently star-forming UFDs. By simulating the Color Magnitude Diagram of Bo\"otes I, and thus take into account the mass-range of the observed stars, we can obtain even tighter constrains on $m_{min}$. By exploiting the 96 stars with measured metallicities ($\rm i < 19$) in the UFDs represented by our model, we demonstrate that: $m_{ch} > 1 \rm M_{\odot}$ or $m_{min} > 0.8 \rm M_{\odot}$ at $99\%$ confidence level. This means that a present day IMF for PopIII stars is excluded by our model, and a top-heavy PopIII IMF is strongly favoured. We can limit $m_{min} > 0.8 \rm M_{\odot}$ independent of the PopIII IMF shape by targeting the four UFDs Bo\"otes I, Hercules, Leo IV and Eridanus II with future generation instruments, such as ELT/MOSAIC ($\rm i < 25$), which can provide samples of >10\,000 stars.

==> include_tex/colors.tex <==

% workaround for colors starging with f
\makeatletter
\def\@hex@@Hex#1%
 {\if a#1A\else \if b#1B\else \if c#1C\else \if d#1D\else
  \if e#1E\else \if f#1F\else #1\fi\fi\fi\fi\fi\fi \@hex@Hex}
\makeatother

\definecolor{apcolor}{HTML}{b3003b}
\definecolor{cbcolor}{HTML}{ff0f00}
\definecolor{afcolor}{HTML}{b3443c}
\definecolor{ddcolor}{HTML}{077a2f}
\definecolor{vgcolor}{HTML}{8F00FF}

\newcommand{\AP}[1]{{\bf \color{apcolor} AP: #1}}
\newcommand{\AF}[1]{{\bf \color{afcolor} AF: #1}}
\newcommand{\VG}[1]{{\bf \color{vgcolor} VG: #1}}


==> include_tex/definizioni.tex <==
\def\be{\begin{equation}} 
\def\ee{\end{equation}} 
\def\ba{\begin{eqnarray}} 
\def\ea{\end{eqnarray}} 
\def\erfc{\rm {erfc}} 
\def\bbf{\bf} 
\def\mpc{\,{\rm {Mpc}}}
\def\mpch{\,h^{-1}{\rm {Mpc}}} 
\def\kms{\,{\rm {km\, s^{-1}}}} 
\def\cc{\,{\rm {cm^{-3}}}} 
\def\msun{{\Msun}} 
\def\vcir{{v_c}}  
\def\dt{{\Delta t}}  
\def\Gyr{{\,\rm Gyr}} 
\def\etal{{\it et al.~}}  
\def\Hm{${\rm {H^-}}\,\,$}  
%\def\HH{${\rm {H_2}}\,\,$}
\def\HH{${\rm {H_2}}$}
\def\HHp{${\rm {H_2^+}}\,\,$} 
\def\sngg{SN$_{\gamma\gamma}$~}  
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{\esc}} 
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\HeI{\hbox{He~$\scriptstyle\rm I\ $}} 
\def\HeII{\hbox{He~$\scriptstyle\rm II\ $}} 
\def\HeIII{\hbox{He~$\scriptstyle\rm III\ $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV\ $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV\ $}} 
\def\OVI{\hbox{O~$\scriptstyle\rm VI\ $}} \def\nHI{{\rm HI}} 
\def\nCIV{{\rm CIV}} \def\nOVI{{\rm OVI}} \def\nH{{\rm H}} 
\def\nHII{{\rm HII}} \def\nHe{{\rm He}} \def\nHeI{{\rm HeI}} 
\def\nHeII{{\rm HeII}} \def\nHeIII{{\rm HeIII}} \def\erg{{\rm erg}} 
\def\sr{{\rm sr}} \def\hz{{\rm Hz}} \def\cm{${\rm cm}$} 
\def\nhi{{N_{\rm HI}}} \def\sec{{\rm s}} 
\def\sigmaba{\sigma_8/usr/local/lib/tex/inputs/latex/styles} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} \def\gtsima{$\; \buildrel > \over 
\sim \;$} \def\ltsima{$\; \buildrel < \over \sim \;$} \def\prosima{$\; 
\buildrel \propto \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} \def\la{\lsim} \def\ga{\gsim} 
\def\ie{{\frenchspacing\it i.e. }} \def\eg{{\frenchspacing\it e.g. }} 
 \def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} 
\def\la{\lsim} 
\def\ga{\gsim} 
\def\de{{\rm d}}
\def\del{\partial}
\def\zcr{Z_{\rm cr}} 
\def\ekin{\mbox{\cal E}_{\rm kin}} 
\def\ekin{{\cal E}_{\rm kin}} 
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{esc}} 
\def\Lya{Ly$\alpha$~} 
\def\sngg{SN-e$^{\pm}$~} 
\def\snggo{SN-e$^{\pm}$} 
\def\msun{\,{\rm \Msun}} 
\def\ie{{\frenchspacing\it i.e., }} 
\def\eg{{\frenchspacing\it e.g., }} 
\def\E3{{\cal E}_{\rm g}^{III}} 
\def\Eunit{\times10^{51} {\rm erg} \, \Msun^{-1}} 
\def\sEunit{10^{51} {\rm erg} \, \Msun^{-1}} 
\def\ozs{\Omega_Z^{sfh}} 
\def\ozo{\Omega_Z^{obs}} 
\def\Onot{\Omega_0} 
\def\Msun{\rm M_\odot}
\def\Zsun{\rm Z_\odot}
\def\rvir{r_{vir}}
\def\rvir{r_{vir}}
\def\vvir{v_{vir}} 
\def\mvir{M_{vir}} 
\def\Tvir{T_{vir}} 
\def\r12{r_{1/2}} 
\def\x12{x_{1/2}} 
\def\v12{v_{1/2}}
\def\ftd{F_{T,D}}
\def\Msf{M_{sf}}



% element astro-like
\def\HI{\hbox{H~$\scriptstyle\rm I $~}}
\def\HII{\hbox{H~$\scriptstyle\rm II $~}}
\def\HeI{\hbox{He~$\scriptstyle\rm I $~}}
\def\HeII{\hbox{He~$\scriptstyle\rm II $~}}
\def\HeIII{\hbox{He~$\scriptstyle\rm III $~}}
%
%\def\CIIion{\hbox{C~$\scriptstyle\rm II $}}
%\def\OIion{\hbox{O~$\scriptstyle\rm I $}}
%\def\OIIIion{\hbox{O~$\scriptstyle\rm III $}}
%\def\NIIion{\hbox{O~$\scriptstyle\rm II $}}
%
\def\CIIion{${\rm C}^{+}$}
\def\OIIIion{${\rm O}^{++}$}
\def\NIIion{${\rm N}^{+}$}

% FIR emission lines
\def\CII{\hbox{[C~$\scriptstyle\rm II $]}}
\def\OI{\hbox{[O~$\scriptstyle\rm I $]}} 
\def\OIII{\hbox{[O~$\scriptstyle\rm III $]}} 
\def\NII{\hbox{[N~$\scriptstyle\rm II $]}}

% absorption lines
\def\MGII{\hbox{Mg~$\scriptstyle\rm II $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV $}}
\def\SiI{\hbox{Si~$\scriptstyle\rm I $}}
\def\SII{\hbox{Si~$\scriptstyle\rm II $}} 
\def\NIIa{\hbox{N~$\scriptstyle\rm IIa $}} 

\def\red{\color{red}}
\def\green{\color{green}}
\def\cyan{\color{cyan}}

% mnras style for code names
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}
\newcommand{\quotes}[1]{``#1''}
\newcommand{\quotesing}[1]{`#1'}

% cosmo
\def\vir{\rm vir}
\def\halo{\rm h}
\def\cent{\rm c}
\def\rvir{r_{\vir}}
\def\zlos{\langle Z\rangle}
%
\def\diinu{\Delta I_{\nu}\slash I_{\nu}}
\def\diiDnu{\Delta I\slash I}
\def\mujb{\mu {\rm Jy}/{\rm beam}}

% math
\def\gt{$>$}

% chemistry
\def\nh2{n_{\rm H2}}
\def\fh2{f_{\rm H2}}
\def\fhp{f_{\rm H+}}
\def\Hp{${\rm H}^{+}$}
\def\dust{\mathcal{D}}
\def\mp{m_{\rm p}}

% units
\def\arcsec{^{\prime\prime}}
\def\angstrom{\textrm{A\kern -1.3ex\raisebox{0.6ex}{$^\circ$}}}
\def\myr{\rm Myr}
\def\mum{\mu{\rm m}}
% solar stuff
\def\msun{{\rm M}_{\odot}}
\def\zsun{{\rm Z}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
\def\dsun{\dust_{\odot}}
%
\def\cc{{\rm cm}^{-3}}
\def\colcm{{\rm cm}^{-2}}
%
\def\msunyr{\msun\,{\rm yr}^{-1}}
\def\surfd{\msun\,{\rm kpc}^{-2}}
\def\surfsfr{\msun\,{\rm yr}^{-1}\,{\rm kpc}^{-2}}
\def\surfdpc{\msun\,{\rm pc}^{-2}}
\def\surfl{\lsun\,{\rm kpc}^{-2}}
\def\voldpc{\msun\,{\rm pc}^{-3}}
%
\def\kpc{{\rm kpc}}
\def\SFR{{\rm SFR}}

%lum and ions
\def\SCII{\Sigma_{\rm [CII]}}
\def\SOIII{\Sigma_{\rm [OIII]}}
\def\SNII{\Sigma_{\rm [NII]}}
\def\SigmaCII{\Sigma_{\rm C+}}
\def\SigmaOIII{\Sigma_{\rm O++}}
\def\SigmaNII{\Sigma_{\rm N+}}
% additional convenience stuff
\def\sigmasfr{\dot{\Sigma}_{\star}}

% names shortcuts
\def\althaea{Alth{\ae}a}
\def\highz{$\mbox{high-}z$~}
